Min-Path-Tracing: A Diffraction Aware Alternative to Image Method in Ray Tracing

For more than twenty years, Ray Tracing methods have continued to improve on both accuracy and computational time aspects. However, most state-of-the-art image-based ray tracers still rely on a description of the environment that only contains planar surfaces. They are also limited by the number of diffractions they can simulate. We present Min-Path-Tracing (MPT), an alternative to the image method that can handle diffractions seamlessly, while also leveraging the possibility to use different geometries for surfaces or edges, such as parabolic mirrors. MPT uses implicit representations of objects to write the path finding challenge as a minimization problem. We further show that multiple diffractions can be important in some situations, which MPT is capable to simulate without increasing neither the computational nor the implementation complexity.

==> colors.tex <==
\definecolor{Accent3qual1}{RGB}{127,201,127}
\definecolor{Accent3qual2}{RGB}{190,174,212}
\definecolor{Accent3qual3}{RGB}{253,192,134}
\definecolor{Accent5qual1}{RGB}{127,201,127}
\definecolor{Accent5qual2}{RGB}{190,174,212}
\definecolor{Accent5qual3}{RGB}{253,192,134}
\definecolor{Accent5qual4}{RGB}{255,255,153}
\definecolor{Accent5qual5}{RGB}{56,108,176}
\definecolor{Accent7qual1}{RGB}{127,201,127}
\definecolor{Accent7qual2}{RGB}{190,174,212}
\definecolor{Accent7qual3}{RGB}{253,192,134}
\definecolor{Accent7qual4}{RGB}{255,255,153}
\definecolor{Accent7qual5}{RGB}{56,108,176}
\definecolor{Accent7qual6}{RGB}{240,2,127}
\definecolor{Accent7qual7}{RGB}{191,91,23}
\definecolor{Blues3seq1}{RGB}{222,235,247}
\definecolor{Blues3seq2}{RGB}{158,202,225}
\definecolor{Blues3seq3}{RGB}{49,130,189}
\definecolor{Blues5seq1}{RGB}{239,243,255}
\definecolor{Blues5seq2}{RGB}{189,215,231}
\definecolor{Blues5seq3}{RGB}{107,174,214}
\definecolor{Blues5seq4}{RGB}{49,130,189}
\definecolor{Blues5seq5}{RGB}{8,81,156}
\definecolor{Blues7seq1}{RGB}{239,243,255}
\definecolor{Blues7seq2}{RGB}{198,219,239}
\definecolor{Blues7seq3}{RGB}{158,202,225}
\definecolor{Blues7seq4}{RGB}{107,174,214}
\definecolor{Blues7seq5}{RGB}{66,146,198}
\definecolor{Blues7seq6}{RGB}{33,113,181}
\definecolor{Blues7seq7}{RGB}{8,69,148}
\definecolor{Blues9seq1}{RGB}{247,251,255}
\definecolor{Blues9seq2}{RGB}{222,235,247}
\definecolor{Blues9seq3}{RGB}{198,219,239}
\definecolor{Blues9seq4}{RGB}{158,202,225}
\definecolor{Blues9seq5}{RGB}{107,174,214}
\definecolor{Blues9seq6}{RGB}{66,146,198}
\definecolor{Blues9seq7}{RGB}{33,113,181}
\definecolor{Blues9seq8}{RGB}{8,81,156}
\definecolor{Blues9seq9}{RGB}{8,48,107}
\definecolor{BrBG4div1}{RGB}{166,97,26}
\definecolor{BrBG4div2}{RGB}{223,194,125}
\definecolor{BrBG4div3}{RGB}{128,205,193}
\definecolor{BrBG4div4}{RGB}{1,133,113}
\definecolor{BrBG6div1}{RGB}{140,81,10}
\definecolor{BrBG6div2}{RGB}{216,179,101}
\definecolor{BrBG6div3}{RGB}{246,232,195}
\definecolor{BrBG6div4}{RGB}{199,234,229}
\definecolor{BrBG6div5}{RGB}{90,180,172}
\definecolor{BrBG6div6}{RGB}{1,102,94}
\definecolor{BrBG8div1}{RGB}{140,81,10}
\definecolor{BrBG8div2}{RGB}{191,129,45}
\definecolor{BrBG8div3}{RGB}{223,194,125}
\definecolor{BrBG8div4}{RGB}{246,232,195}
\definecolor{BrBG8div5}{RGB}{199,234,229}
\definecolor{BrBG8div6}{RGB}{128,205,193}
\definecolor{BrBG8div7}{RGB}{53,151,143}
\definecolor{BrBG8div8}{RGB}{1,102,94}
\definecolor{BrBG10div1}{RGB}{84,48,5}
\definecolor{BrBG10div2}{RGB}{140,81,10}
\definecolor{BrBG10div3}{RGB}{191,129,45}
\definecolor{BrBG10div4}{RGB}{223,194,125}
\definecolor{BrBG10div5}{RGB}{246,232,195}
\definecolor{BrBG10div6}{RGB}{199,234,229}
\definecolor{BrBG10div7}{RGB}{128,205,193}
\definecolor{BrBG10div8}{RGB}{53,151,143}
\definecolor{BrBG10div9}{RGB}{1,102,94}
\definecolor{BrBG10div10}{RGB}{0,60,48}
\definecolor{BuGn3seq1}{RGB}{229,245,249}
\definecolor{BuGn3seq2}{RGB}{153,216,201}
\definecolor{BuGn3seq3}{RGB}{44,162,95}
\definecolor{BuGn5seq1}{RGB}{237,248,251}
\definecolor{BuGn5seq2}{RGB}{178,226,226}
\definecolor{BuGn5seq3}{RGB}{102,194,164}
\definecolor{BuGn5seq4}{RGB}{44,162,95}
\definecolor{BuGn5seq5}{RGB}{0,109,44}
\definecolor{BuGn7seq1}{RGB}{237,248,251}
\definecolor{BuGn7seq2}{RGB}{204,236,230}
\definecolor{BuGn7seq3}{RGB}{153,216,201}
\definecolor{BuGn7seq4}{RGB}{102,194,164}
\definecolor{BuGn7seq5}{RGB}{65,174,118}
\definecolor{BuGn7seq6}{RGB}{35,139,69}
\definecolor{BuGn7seq7}{RGB}{0,88,36}
\definecolor{BuGn9seq1}{RGB}{247,252,253}
\definecolor{BuGn9seq2}{RGB}{229,245,249}
\definecolor{BuGn9seq3}{RGB}{204,236,230}
\definecolor{BuGn9seq4}{RGB}{153,216,201}
\definecolor{BuGn9seq5}{RGB}{102,194,164}
\definecolor{BuGn9seq6}{RGB}{65,174,118}
\definecolor{BuGn9seq7}{RGB}{35,139,69}
\definecolor{BuGn9seq8}{RGB}{0,109,44}
\definecolor{BuGn9seq9}{RGB}{0,68,27}
\definecolor{BuPu4seq1}{RGB}{237,248,251}
\definecolor{BuPu4seq2}{RGB}{179,205,227}
\definecolor{BuPu4seq3}{RGB}{140,150,198}
\definecolor{BuPu4seq4}{RGB}{136,65,157}
\definecolor{BuPu6seq1}{RGB}{237,248,251}
\definecolor{BuPu6seq2}{RGB}{191,211,230}
\definecolor{BuPu6seq3}{RGB}{158,188,218}
\definecolor{BuPu6seq4}{RGB}{140,150,198}
\definecolor{BuPu6seq5}{RGB}{136,86,167}
\definecolor{BuPu6seq6}{RGB}{129,15,124}
\definecolor{BuPu8seq1}{RGB}{247,252,253}
\definecolor{BuPu8seq2}{RGB}{224,236,244}
\definecolor{BuPu8seq3}{RGB}{191,211,230}
\definecolor{BuPu8seq4}{RGB}{158,188,218}
\definecolor{BuPu8seq5}{RGB}{140,150,198}
\definecolor{BuPu8seq6}{RGB}{140,107,177}
\definecolor{BuPu8seq7}{RGB}{136,65,157}
\definecolor{BuPu8seq8}{RGB}{110,1,107}
\definecolor{Dark23qual1}{RGB}{27,158,119}
\definecolor{Dark23qual2}{RGB}{217,95,2}
\definecolor{Dark23qual3}{RGB}{117,112,179}
\definecolor{Dark25qual1}{RGB}{27,158,119}
\definecolor{Dark25qual2}{RGB}{217,95,2}
\definecolor{Dark25qual3}{RGB}{117,112,179}
\definecolor{Dark25qual4}{RGB}{231,41,138}
\definecolor{Dark25qual5}{RGB}{102,166,30}
\definecolor{Dark27qual1}{RGB}{27,158,119}
\definecolor{Dark27qual2}{RGB}{217,95,2}
\definecolor{Dark27qual3}{RGB}{117,112,179}
\definecolor{Dark27qual4}{RGB}{231,41,138}
\definecolor{Dark27qual5}{RGB}{102,166,30}
\definecolor{Dark27qual6}{RGB}{230,171,2}
\definecolor{Dark27qual7}{RGB}{166,118,29}
\definecolor{GnBu3seq1}{RGB}{224,243,219}
\definecolor{GnBu3seq2}{RGB}{168,221,181}
\definecolor{GnBu3seq3}{RGB}{67,162,202}
\definecolor{GnBu5seq1}{RGB}{240,249,232}
\definecolor{GnBu5seq2}{RGB}{186,228,188}
\definecolor{GnBu5seq3}{RGB}{123,204,196}
\definecolor{GnBu5seq4}{RGB}{67,162,202}
\definecolor{GnBu5seq5}{RGB}{8,104,172}
\definecolor{GnBu7seq1}{RGB}{240,249,232}
\definecolor{GnBu7seq2}{RGB}{204,235,197}
\definecolor{GnBu7seq3}{RGB}{168,221,181}
\definecolor{GnBu7seq4}{RGB}{123,204,196}
\definecolor{GnBu7seq5}{RGB}{78,179,211}
\definecolor{GnBu7seq6}{RGB}{43,140,190}
\definecolor{GnBu7seq7}{RGB}{8,88,158}
\definecolor{GnBu9seq1}{RGB}{247,252,240}
\definecolor{GnBu9seq2}{RGB}{224,243,219}
\definecolor{GnBu9seq3}{RGB}{204,235,197}
\definecolor{GnBu9seq4}{RGB}{168,221,181}
\definecolor{GnBu9seq5}{RGB}{123,204,196}
\definecolor{GnBu9seq6}{RGB}{78,179,211}
\definecolor{GnBu9seq7}{RGB}{43,140,190}
\definecolor{GnBu9seq8}{RGB}{8,104,172}
\definecolor{GnBu9seq9}{RGB}{8,64,129}
\definecolor{Greens4seq1}{RGB}{237,248,233}
\definecolor{Greens4seq2}{RGB}{186,228,179}
\definecolor{Greens4seq3}{RGB}{116,196,118}
\definecolor{Greens4seq4}{RGB}{35,139,69}
\definecolor{Greens6seq1}{RGB}{237,248,233}
\definecolor{Greens6seq2}{RGB}{199,233,192}
\definecolor{Greens6seq3}{RGB}{161,217,155}
\definecolor{Greens6seq4}{RGB}{116,196,118}
\definecolor{Greens6seq5}{RGB}{49,163,84}
\definecolor{Greens6seq6}{RGB}{0,109,44}
\definecolor{Greens8seq1}{RGB}{247,252,245}
\definecolor{Greens8seq2}{RGB}{229,245,224}
\definecolor{Greens8seq3}{RGB}{199,233,192}
\definecolor{Greens8seq4}{RGB}{161,217,155}
\definecolor{Greens8seq5}{RGB}{116,196,118}
\definecolor{Greens8seq6}{RGB}{65,171,93}
\definecolor{Greens8seq7}{RGB}{35,139,69}
\definecolor{Greens8seq8}{RGB}{0,90,50}
\definecolor{Greys3seq1}{RGB}{240,240,240}
\definecolor{Greys3seq2}{RGB}{189,189,189}
\definecolor{Greys3seq3}{RGB}{99,99,99}
\definecolor{Greys5seq1}{RGB}{247,247,247}
\definecolor{Greys5seq2}{RGB}{204,204,204}
\definecolor{Greys5seq3}{RGB}{150,150,150}
\definecolor{Greys5seq4}{RGB}{99,99,99}
\definecolor{Greys5seq5}{RGB}{37,37,37}
\definecolor{Greys7seq1}{RGB}{247,247,247}
\definecolor{Greys7seq2}{RGB}{217,217,217}
\definecolor{Greys7seq3}{RGB}{189,189,189}
\definecolor{Greys7seq4}{RGB}{150,150,150}
\definecolor{Greys7seq5}{RGB}{115,115,115}
\definecolor{Greys7seq6}{RGB}{82,82,82}
\definecolor{Greys7seq7}{RGB}{37,37,37}
\definecolor{Greys9seq1}{RGB}{255,255,255}
\definecolor{Greys9seq2}{RGB}{240,240,240}
\definecolor{Greys9seq3}{RGB}{217,217,217}
\definecolor{Greys9seq4}{RGB}{189,189,189}
\definecolor{Greys9seq5}{RGB}{150,150,150}
\definecolor{Greys9seq6}{RGB}{115,115,115}
\definecolor{Greys9seq7}{RGB}{82,82,82}
\definecolor{Greys9seq8}{RGB}{37,37,37}
\definecolor{Greys9seq9}{RGB}{0,0,0}
\definecolor{Oranges4seq1}{RGB}{254,237,222}
\definecolor{Oranges4seq2}{RGB}{253,190,133}
\definecolor{Oranges4seq3}{RGB}{253,141,60}
\definecolor{Oranges4seq4}{RGB}{217,71,1}
\definecolor{Oranges6seq1}{RGB}{254,237,222}
\definecolor{Oranges6seq2}{RGB}{253,208,162}
\definecolor{Oranges6seq3}{RGB}{253,174,107}
\definecolor{Oranges6seq4}{RGB}{253,141,60}
\definecolor{Oranges6seq5}{RGB}{230,85,13}
\definecolor{Oranges6seq6}{RGB}{166,54,3}
\definecolor{Oranges8seq1}{RGB}{255,245,235}
\definecolor{Oranges8seq2}{RGB}{254,230,206}
\definecolor{Oranges8seq3}{RGB}{253,208,162}
\definecolor{Oranges8seq4}{RGB}{253,174,107}
\definecolor{Oranges8seq5}{RGB}{253,141,60}
\definecolor{Oranges8seq6}{RGB}{241,105,19}
\definecolor{Oranges8seq7}{RGB}{217,72,1}
\definecolor{Oranges8seq8}{RGB}{140,45,4}
\definecolor{OrRd3seq1}{RGB}{254,232,200}
\definecolor{OrRd3seq2}{RGB}{253,187,132}
\definecolor{OrRd3seq3}{RGB}{227,74,51}
\definecolor{OrRd5seq1}{RGB}{254,240,217}
\definecolor{OrRd5seq2}{RGB}{253,204,138}
\definecolor{OrRd5seq3}{RGB}{252,141,89}
\definecolor{OrRd5seq4}{RGB}{227,74,51}
\definecolor{OrRd5seq5}{RGB}{179,0,0}
\definecolor{OrRd7seq1}{RGB}{254,240,217}
\definecolor{OrRd7seq2}{RGB}{253,212,158}
\definecolor{OrRd7seq3}{RGB}{253,187,132}
\definecolor{OrRd7seq4}{RGB}{252,141,89}
\definecolor{OrRd7seq5}{RGB}{239,101,72}
\definecolor{OrRd7seq6}{RGB}{215,48,31}
\definecolor{OrRd7seq7}{RGB}{153,0,0}
\definecolor{OrRd9seq1}{RGB}{255,247,236}
\definecolor{OrRd9seq2}{RGB}{254,232,200}
\definecolor{OrRd9seq3}{RGB}{253,212,158}
\definecolor{OrRd9seq4}{RGB}{253,187,132}
\definecolor{OrRd9seq5}{RGB}{252,141,89}
\definecolor{OrRd9seq6}{RGB}{239,101,72}
\definecolor{OrRd9seq7}{RGB}{215,48,31}
\definecolor{OrRd9seq8}{RGB}{179,0,0}
\definecolor{OrRd9seq9}{RGB}{127,0,0}
\definecolor{Paired4qual1}{RGB}{166,206,227}
\definecolor{Paired4qual2}{RGB}{31,120,180}
\definecolor{Paired4qual3}{RGB}{178,223,138}
\definecolor{Paired4qual4}{RGB}{51,160,44}
\definecolor{Paired6qual1}{RGB}{166,206,227}
\definecolor{Paired6qual2}{RGB}{31,120,180}
\definecolor{Paired6qual3}{RGB}{178,223,138}
\definecolor{Paired6qual4}{RGB}{51,160,44}
\definecolor{Paired6qual5}{RGB}{251,154,153}
\definecolor{Paired6qual6}{RGB}{227,26,28}
\definecolor{Paired8qual1}{RGB}{166,206,227}
\definecolor{Paired8qual2}{RGB}{31,120,180}
\definecolor{Paired8qual3}{RGB}{178,223,138}
\definecolor{Paired8qual4}{RGB}{51,160,44}
\definecolor{Paired8qual5}{RGB}{251,154,153}
\definecolor{Paired8qual6}{RGB}{227,26,28}
\definecolor{Paired8qual7}{RGB}{253,191,111}
\definecolor{Paired8qual8}{RGB}{255,127,0}
\definecolor{Paired10qual1}{RGB}{166,206,227}
\definecolor{Paired10qual2}{RGB}{31,120,180}
\definecolor{Paired10qual3}{RGB}{178,223,138}
\definecolor{Paired10qual4}{RGB}{51,160,44}
\definecolor{Paired10qual5}{RGB}{251,154,153}
\definecolor{Paired10qual6}{RGB}{227,26,28}
\definecolor{Paired10qual7}{RGB}{253,191,111}
\definecolor{Paired10qual8}{RGB}{255,127,0}
\definecolor{Paired10qual9}{RGB}{202,178,214}
\definecolor{Paired10qual10}{RGB}{106,61,154}
\definecolor{Paired12qual1}{RGB}{166,206,227}
\definecolor{Paired12qual2}{RGB}{31,120,180}
\definecolor{Paired12qual3}{RGB}{178,223,138}
\definecolor{Paired12qual4}{RGB}{51,160,44}
\definecolor{Paired12qual5}{RGB}{251,154,153}
\definecolor{Paired12qual6}{RGB}{227,26,28}
\definecolor{Paired12qual7}{RGB}{253,191,111}
\definecolor{Paired12qual8}{RGB}{255,127,0}
\definecolor{Paired12qual9}{RGB}{202,178,214}
\definecolor{Paired12qual10}{RGB}{106,61,154}
\definecolor{Paired12qual11}{RGB}{255,255,153}
\definecolor{Paired12qual12}{RGB}{177,89,40}
\definecolor{Pastel14qual1}{RGB}{251,180,174}
\definecolor{Pastel14qual2}{RGB}{179,205,227}
\definecolor{Pastel14qual3}{RGB}{204,235,197}
\definecolor{Pastel14qual4}{RGB}{222,203,228}
\definecolor{Pastel16qual1}{RGB}{251,180,174}
\definecolor{Pastel16qual2}{RGB}{179,205,227}
\definecolor{Pastel16qual3}{RGB}{204,235,197}
\definecolor{Pastel16qual4}{RGB}{222,203,228}
\definecolor{Pastel16qual5}{RGB}{254,217,166}
\definecolor{Pastel16qual6}{RGB}{255,255,204}
\definecolor{Pastel18qual1}{RGB}{251,180,174}
\definecolor{Pastel18qual2}{RGB}{179,205,227}
\definecolor{Pastel18qual3}{RGB}{204,235,197}
\definecolor{Pastel18qual4}{RGB}{222,203,228}
\definecolor{Pastel18qual5}{RGB}{254,217,166}
\definecolor{Pastel18qual6}{RGB}{255,255,204}
\definecolor{Pastel18qual7}{RGB}{229,216,189}
\definecolor{Pastel18qual8}{RGB}{253,218,236}
\definecolor{Pastel23qual1}{RGB}{179,226,205}
\definecolor{Pastel23qual2}{RGB}{253,205,172}
\definecolor{Pastel23qual3}{RGB}{203,213,232}
\definecolor{Pastel25qual1}{RGB}{179,226,205}
\definecolor{Pastel25qual2}{RGB}{253,205,172}
\definecolor{Pastel25qual3}{RGB}{203,213,232}
\definecolor{Pastel25qual4}{RGB}{244,202,228}
\definecolor{Pastel25qual5}{RGB}{230,245,201}
\definecolor{Pastel27qual1}{RGB}{179,226,205}
\definecolor{Pastel27qual2}{RGB}{253,205,172}
\definecolor{Pastel27qual3}{RGB}{203,213,232}
\definecolor{Pastel27qual4}{RGB}{244,202,228}
\definecolor{Pastel27qual5}{RGB}{230,245,201}
\definecolor{Pastel27qual6}{RGB}{255,242,174}
\definecolor{Pastel27qual7}{RGB}{241,226,204}
\definecolor{PiYG3div1}{RGB}{233,163,201}
\definecolor{PiYG3div2}{RGB}{247,247,247}
\definecolor{PiYG3div3}{RGB}{161,215,106}
\definecolor{PiYG5div1}{RGB}{208,28,139}
\definecolor{PiYG5div2}{RGB}{241,182,218}
\definecolor{PiYG5div3}{RGB}{247,247,247}
\definecolor{PiYG5div4}{RGB}{184,225,134}
\definecolor{PiYG5div5}{RGB}{77,172,38}
\definecolor{PiYG7div1}{RGB}{197,27,125}
\definecolor{PiYG7div2}{RGB}{233,163,201}
\definecolor{PiYG7div3}{RGB}{253,224,239}
\definecolor{PiYG7div4}{RGB}{247,247,247}
\definecolor{PiYG7div5}{RGB}{230,245,208}
\definecolor{PiYG7div6}{RGB}{161,215,106}
\definecolor{PiYG7div7}{RGB}{77,146,33}
\definecolor{PiYG9div1}{RGB}{197,27,125}
\definecolor{PiYG9div2}{RGB}{222,119,174}
\definecolor{PiYG9div3}{RGB}{241,182,218}
\definecolor{PiYG9div4}{RGB}{253,224,239}
\definecolor{PiYG9div5}{RGB}{247,247,247}
\definecolor{PiYG9div6}{RGB}{230,245,208}
\definecolor{PiYG9div7}{RGB}{184,225,134}
\definecolor{PiYG9div8}{RGB}{127,188,65}
\definecolor{PiYG9div9}{RGB}{77,146,33}
\definecolor{PiYG11div1}{RGB}{142,1,82}
\definecolor{PiYG11div2}{RGB}{197,27,125}
\definecolor{PiYG11div3}{RGB}{222,119,174}
\definecolor{PiYG11div4}{RGB}{241,182,218}
\definecolor{PiYG11div5}{RGB}{253,224,239}
\definecolor{PiYG11div6}{RGB}{247,247,247}
\definecolor{PiYG11div7}{RGB}{230,245,208}
\definecolor{PiYG11div8}{RGB}{184,225,134}
\definecolor{PiYG11div9}{RGB}{127,188,65}
\definecolor{PiYG11div10}{RGB}{77,146,33}
\definecolor{PiYG11div11}{RGB}{39,100,25}
\definecolor{PRGn4div1}{RGB}{123,50,148}
\definecolor{PRGn4div2}{RGB}{194,165,207}
\definecolor{PRGn4div3}{RGB}{166,219,160}
\definecolor{PRGn4div4}{RGB}{0,136,55}
\definecolor{PRGn6div1}{RGB}{118,42,131}
\definecolor{PRGn6div2}{RGB}{175,141,195}
\definecolor{PRGn6div3}{RGB}{231,212,232}
\definecolor{PRGn6div4}{RGB}{217,240,211}
\definecolor{PRGn6div5}{RGB}{127,191,123}
\definecolor{PRGn6div6}{RGB}{27,120,55}
\definecolor{PRGn8div1}{RGB}{118,42,131}
\definecolor{PRGn8div2}{RGB}{153,112,171}
\definecolor{PRGn8div3}{RGB}{194,165,207}
\definecolor{PRGn8div4}{RGB}{231,212,232}
\definecolor{PRGn8div5}{RGB}{217,240,211}
\definecolor{PRGn8div6}{RGB}{166,219,160}
\definecolor{PRGn8div7}{RGB}{90,174,97}
\definecolor{PRGn8div8}{RGB}{27,120,55}
\definecolor{PRGn10div1}{RGB}{64,0,75}
\definecolor{PRGn10div2}{RGB}{118,42,131}
\definecolor{PRGn10div3}{RGB}{153,112,171}
\definecolor{PRGn10div4}{RGB}{194,165,207}
\definecolor{PRGn10div5}{RGB}{231,212,232}
\definecolor{PRGn10div6}{RGB}{217,240,211}
\definecolor{PRGn10div7}{RGB}{166,219,160}
\definecolor{PRGn10div8}{RGB}{90,174,97}
\definecolor{PRGn10div9}{RGB}{27,120,55}
\definecolor{PRGn10div10}{RGB}{0,68,27}
\definecolor{PuBu3seq1}{RGB}{236,231,242}
\definecolor{PuBu3seq2}{RGB}{166,189,219}
\definecolor{PuBu3seq3}{RGB}{43,140,190}
\definecolor{PuBu5seq1}{RGB}{241,238,246}
\definecolor{PuBu5seq2}{RGB}{189,201,225}
\definecolor{PuBu5seq3}{RGB}{116,169,207}
\definecolor{PuBu5seq4}{RGB}{43,140,190}
\definecolor{PuBu5seq5}{RGB}{4,90,141}
\definecolor{PuBu7seq1}{RGB}{241,238,246}
\definecolor{PuBu7seq2}{RGB}{208,209,230}
\definecolor{PuBu7seq3}{RGB}{166,189,219}
\definecolor{PuBu7seq4}{RGB}{116,169,207}
\definecolor{PuBu7seq5}{RGB}{54,144,192}
\definecolor{PuBu7seq6}{RGB}{5,112,176}
\definecolor{PuBu7seq7}{RGB}{3,78,123}
\definecolor{PuBu9seq1}{RGB}{255,247,251}
\definecolor{PuBu9seq2}{RGB}{236,231,242}
\definecolor{PuBu9seq3}{RGB}{208,209,230}
\definecolor{PuBu9seq4}{RGB}{166,189,219}
\definecolor{PuBu9seq5}{RGB}{116,169,207}
\definecolor{PuBu9seq6}{RGB}{54,144,192}
\definecolor{PuBu9seq7}{RGB}{5,112,176}
\definecolor{PuBu9seq8}{RGB}{4,90,141}
\definecolor{PuBu9seq9}{RGB}{2,56,88}
\definecolor{PuBuGn4seq1}{RGB}{246,239,247}
\definecolor{PuBuGn4seq2}{RGB}{189,201,225}
\definecolor{PuBuGn4seq3}{RGB}{103,169,207}
\definecolor{PuBuGn4seq4}{RGB}{2,129,138}
\definecolor{PuBuGn6seq1}{RGB}{246,239,247}
\definecolor{PuBuGn6seq2}{RGB}{208,209,230}
\definecolor{PuBuGn6seq3}{RGB}{166,189,219}
\definecolor{PuBuGn6seq4}{RGB}{103,169,207}
\definecolor{PuBuGn6seq5}{RGB}{28,144,153}
\definecolor{PuBuGn6seq6}{RGB}{1,108,89}
\definecolor{PuBuGn8seq1}{RGB}{255,247,251}
\definecolor{PuBuGn8seq2}{RGB}{236,226,240}
\definecolor{PuBuGn8seq3}{RGB}{208,209,230}
\definecolor{PuBuGn8seq4}{RGB}{166,189,219}
\definecolor{PuBuGn8seq5}{RGB}{103,169,207}
\definecolor{PuBuGn8seq6}{RGB}{54,144,192}
\definecolor{PuBuGn8seq7}{RGB}{2,129,138}
\definecolor{PuBuGn8seq8}{RGB}{1,100,80}
\definecolor{PuOr3div1}{RGB}{241,163,64}
\definecolor{PuOr3div2}{RGB}{247,247,247}
\definecolor{PuOr3div3}{RGB}{153,142,195}
\definecolor{PuOr5div1}{RGB}{230,97,1}
\definecolor{PuOr5div2}{RGB}{253,184,99}
\definecolor{PuOr5div3}{RGB}{247,247,247}
\definecolor{PuOr5div4}{RGB}{178,171,210}
\definecolor{PuOr5div5}{RGB}{94,60,153}
\definecolor{PuOr7div1}{RGB}{179,88,6}
\definecolor{PuOr7div2}{RGB}{241,163,64}
\definecolor{PuOr7div3}{RGB}{254,224,182}
\definecolor{PuOr7div4}{RGB}{247,247,247}
\definecolor{PuOr7div5}{RGB}{216,218,235}
\definecolor{PuOr7div6}{RGB}{153,142,195}
\definecolor{PuOr7div7}{RGB}{84,39,136}
\definecolor{PuOr9div1}{RGB}{179,88,6}
\definecolor{PuOr9div2}{RGB}{224,130,20}
\definecolor{PuOr9div3}{RGB}{253,184,99}
\definecolor{PuOr9div4}{RGB}{254,224,182}
\definecolor{PuOr9div5}{RGB}{247,247,247}
\definecolor{PuOr9div6}{RGB}{216,218,235}
\definecolor{PuOr9div7}{RGB}{178,171,210}
\definecolor{PuOr9div8}{RGB}{128,115,172}
\definecolor{PuOr9div9}{RGB}{84,39,136}
\definecolor{PuOr11div1}{RGB}{127,59,8}
\definecolor{PuOr11div2}{RGB}{179,88,6}
\definecolor{PuOr11div3}{RGB}{224,130,20}
\definecolor{PuOr11div4}{RGB}{253,184,99}
\definecolor{PuOr11div5}{RGB}{254,224,182}
\definecolor{PuOr11div6}{RGB}{247,247,247}
\definecolor{PuOr11div7}{RGB}{216,218,235}
\definecolor{PuOr11div8}{RGB}{178,171,210}
\definecolor{PuOr11div9}{RGB}{128,115,172}
\definecolor{PuOr11div10}{RGB}{84,39,136}
\definecolor{PuOr11div11}{RGB}{45,0,75}
\definecolor{PuRd4seq1}{RGB}{241,238,246}
\definecolor{PuRd4seq2}{RGB}{215,181,216}
\definecolor{PuRd4seq3}{RGB}{223,101,176}
\definecolor{PuRd4seq4}{RGB}{206,18,86}
\definecolor{PuRd6seq1}{RGB}{241,238,246}
\definecolor{PuRd6seq2}{RGB}{212,185,218}
\definecolor{PuRd6seq3}{RGB}{201,148,199}
\definecolor{PuRd6seq4}{RGB}{223,101,176}
\definecolor{PuRd6seq5}{RGB}{221,28,119}
\definecolor{PuRd6seq6}{RGB}{152,0,67}
\definecolor{PuRd8seq1}{RGB}{247,244,249}
\definecolor{PuRd8seq2}{RGB}{231,225,239}
\definecolor{PuRd8seq3}{RGB}{212,185,218}
\definecolor{PuRd8seq4}{RGB}{201,148,199}
\definecolor{PuRd8seq5}{RGB}{223,101,176}
\definecolor{PuRd8seq6}{RGB}{231,41,138}
\definecolor{PuRd8seq7}{RGB}{206,18,86}
\definecolor{PuRd8seq8}{RGB}{145,0,63}
\definecolor{Purples3seq1}{RGB}{239,237,245}
\definecolor{Purples3seq2}{RGB}{188,189,220}
\definecolor{Purples3seq3}{RGB}{117,107,177}
\definecolor{Purples5seq1}{RGB}{242,240,247}
\definecolor{Purples5seq2}{RGB}{203,201,226}
\definecolor{Purples5seq3}{RGB}{158,154,200}
\definecolor{Purples5seq4}{RGB}{117,107,177}
\definecolor{Purples5seq5}{RGB}{84,39,143}
\definecolor{Purples7seq1}{RGB}{242,240,247}
\definecolor{Purples7seq2}{RGB}{218,218,235}
\definecolor{Purples7seq3}{RGB}{188,189,220}
\definecolor{Purples7seq4}{RGB}{158,154,200}
\definecolor{Purples7seq5}{RGB}{128,125,186}
\definecolor{Purples7seq6}{RGB}{106,81,163}
\definecolor{Purples7seq7}{RGB}{74,20,134}
\definecolor{Purples9seq1}{RGB}{252,251,253}
\definecolor{Purples9seq2}{RGB}{239,237,245}
\definecolor{Purples9seq3}{RGB}{218,218,235}
\definecolor{Purples9seq4}{RGB}{188,189,220}
\definecolor{Purples9seq5}{RGB}{158,154,200}
\definecolor{Purples9seq6}{RGB}{128,125,186}
\definecolor{Purples9seq7}{RGB}{106,81,163}
\definecolor{Purples9seq8}{RGB}{84,39,143}
\definecolor{Purples9seq9}{RGB}{63,0,125}
\definecolor{RdBu4div1}{RGB}{202,0,32}
\definecolor{RdBu4div2}{RGB}{244,165,130}
\definecolor{RdBu4div3}{RGB}{146,197,222}
\definecolor{RdBu4div4}{RGB}{5,113,176}
\definecolor{RdBu6div1}{RGB}{178,24,43}
\definecolor{RdBu6div2}{RGB}{239,138,98}
\definecolor{RdBu6div3}{RGB}{253,219,199}
\definecolor{RdBu6div4}{RGB}{209,229,240}
\definecolor{RdBu6div5}{RGB}{103,169,207}
\definecolor{RdBu6div6}{RGB}{33,102,172}
\definecolor{RdBu8div1}{RGB}{178,24,43}
\definecolor{RdBu8div2}{RGB}{214,96,77}
\definecolor{RdBu8div3}{RGB}{244,165,130}
\definecolor{RdBu8div4}{RGB}{253,219,199}
\definecolor{RdBu8div5}{RGB}{209,229,240}
\definecolor{RdBu8div6}{RGB}{146,197,222}
\definecolor{RdBu8div7}{RGB}{67,147,195}
\definecolor{RdBu8div8}{RGB}{33,102,172}
\definecolor{RdBu10div1}{RGB}{103,0,31}
\definecolor{RdBu10div2}{RGB}{178,24,43}
\definecolor{RdBu10div3}{RGB}{214,96,77}
\definecolor{RdBu10div4}{RGB}{244,165,130}
\definecolor{RdBu10div5}{RGB}{253,219,199}
\definecolor{RdBu10div6}{RGB}{209,229,240}
\definecolor{RdBu10div7}{RGB}{146,197,222}
\definecolor{RdBu10div8}{RGB}{67,147,195}
\definecolor{RdBu10div9}{RGB}{33,102,172}
\definecolor{RdBu10div10}{RGB}{5,48,97}
\definecolor{RdGy3div1}{RGB}{239,138,98}
\definecolor{RdGy3div2}{RGB}{255,255,255}
\definecolor{RdGy3div3}{RGB}{153,153,153}
\definecolor{RdGy5div1}{RGB}{202,0,32}
\definecolor{RdGy5div2}{RGB}{244,165,130}
\definecolor{RdGy5div3}{RGB}{255,255,255}
\definecolor{RdGy5div4}{RGB}{186,186,186}
\definecolor{RdGy5div5}{RGB}{64,64,64}
\definecolor{RdGy7div1}{RGB}{178,24,43}
\definecolor{RdGy7div2}{RGB}{239,138,98}
\definecolor{RdGy7div3}{RGB}{253,219,199}
\definecolor{RdGy7div4}{RGB}{255,255,255}
\definecolor{RdGy7div5}{RGB}{224,224,224}
\definecolor{RdGy7div6}{RGB}{153,153,153}
\definecolor{RdGy7div7}{RGB}{77,77,77}
\definecolor{RdGy9div1}{RGB}{178,24,43}
\definecolor{RdGy9div2}{RGB}{214,96,77}
\definecolor{RdGy9div3}{RGB}{244,165,130}
\definecolor{RdGy9div4}{RGB}{253,219,199}
\definecolor{RdGy9div5}{RGB}{255,255,255}
\definecolor{RdGy9div6}{RGB}{224,224,224}
\definecolor{RdGy9div7}{RGB}{186,186,186}
\definecolor{RdGy9div8}{RGB}{135,135,135}
\definecolor{RdGy9div9}{RGB}{77,77,77}
\definecolor{RdGy11div1}{RGB}{103,0,31}
\definecolor{RdGy11div2}{RGB}{178,24,43}
\definecolor{RdGy11div3}{RGB}{214,96,77}
\definecolor{RdGy11div4}{RGB}{244,165,130}
\definecolor{RdGy11div5}{RGB}{253,219,199}
\definecolor{RdGy11div6}{RGB}{255,255,255}
\definecolor{RdGy11div7}{RGB}{224,224,224}
\definecolor{RdGy11div8}{RGB}{186,186,186}
\definecolor{RdGy11div9}{RGB}{135,135,135}
\definecolor{RdGy11div10}{RGB}{77,77,77}
\definecolor{RdGy11div11}{RGB}{26,26,26}
\definecolor{RdPu4seq1}{RGB}{254,235,226}
\definecolor{RdPu4seq2}{RGB}{251,180,185}
\definecolor{RdPu4seq3}{RGB}{247,104,161}
\definecolor{RdPu4seq4}{RGB}{174,1,126}
\definecolor{RdPu6seq1}{RGB}{254,235,226}
\definecolor{RdPu6seq2}{RGB}{252,197,192}
\definecolor{RdPu6seq3}{RGB}{250,159,181}
\definecolor{RdPu6seq4}{RGB}{247,104,161}
\definecolor{RdPu6seq5}{RGB}{197,27,138}
\definecolor{RdPu6seq6}{RGB}{122,1,119}
\definecolor{RdPu8seq1}{RGB}{255,247,243}
\definecolor{RdPu8seq2}{RGB}{253,224,221}
\definecolor{RdPu8seq3}{RGB}{252,197,192}
\definecolor{RdPu8seq4}{RGB}{250,159,181}
\definecolor{RdPu8seq5}{RGB}{247,104,161}
\definecolor{RdPu8seq6}{RGB}{221,52,151}
\definecolor{RdPu8seq7}{RGB}{174,1,126}
\definecolor{RdPu8seq8}{RGB}{122,1,119}
\definecolor{Reds3seq1}{RGB}{254,224,210}
\definecolor{Reds3seq2}{RGB}{252,146,114}
\definecolor{Reds3seq3}{RGB}{222,45,38}
\definecolor{Reds5seq1}{RGB}{254,229,217}
\definecolor{Reds5seq2}{RGB}{252,174,145}
\definecolor{Reds5seq3}{RGB}{251,106,74}
\definecolor{Reds5seq4}{RGB}{222,45,38}
\definecolor{Reds5seq5}{RGB}{165,15,21}
\definecolor{Reds7seq1}{RGB}{254,229,217}
\definecolor{Reds7seq2}{RGB}{252,187,161}
\definecolor{Reds7seq3}{RGB}{252,146,114}
\definecolor{Reds7seq4}{RGB}{251,106,74}
\definecolor{Reds7seq5}{RGB}{239,59,44}
\definecolor{Reds7seq6}{RGB}{203,24,29}
\definecolor{Reds7seq7}{RGB}{153,0,13}
\definecolor{Reds9seq1}{RGB}{255,245,240}
\definecolor{Reds9seq2}{RGB}{254,224,210}
\definecolor{Reds9seq3}{RGB}{252,187,161}
\definecolor{Reds9seq4}{RGB}{252,146,114}
\definecolor{Reds9seq5}{RGB}{251,106,74}
\definecolor{Reds9seq6}{RGB}{239,59,44}
\definecolor{Reds9seq7}{RGB}{203,24,29}
\definecolor{Reds9seq8}{RGB}{165,15,21}
\definecolor{Reds9seq9}{RGB}{103,0,13}
\definecolor{RdYlBu4div1}{RGB}{215,25,28}
\definecolor{RdYlBu4div2}{RGB}{253,174,97}
\definecolor{RdYlBu4div3}{RGB}{171,217,233}
\definecolor{RdYlBu4div4}{RGB}{44,123,182}
\definecolor{RdYlBu6div1}{RGB}{215,48,39}
\definecolor{RdYlBu6div2}{RGB}{252,141,89}
\definecolor{RdYlBu6div3}{RGB}{254,224,144}
\definecolor{RdYlBu6div4}{RGB}{224,243,248}
\definecolor{RdYlBu6div5}{RGB}{145,191,219}
\definecolor{RdYlBu6div6}{RGB}{69,117,180}
\definecolor{RdYlBu8div1}{RGB}{215,48,39}
\definecolor{RdYlBu8div2}{RGB}{244,109,67}
\definecolor{RdYlBu8div3}{RGB}{253,174,97}
\definecolor{RdYlBu8div4}{RGB}{254,224,144}
\definecolor{RdYlBu8div5}{RGB}{224,243,248}
\definecolor{RdYlBu8div6}{RGB}{171,217,233}
\definecolor{RdYlBu8div7}{RGB}{116,173,209}
\definecolor{RdYlBu8div8}{RGB}{69,117,180}
\definecolor{RdYlBu10div1}{RGB}{165,0,38}
\definecolor{RdYlBu10div2}{RGB}{215,48,39}
\definecolor{RdYlBu10div3}{RGB}{244,109,67}
\definecolor{RdYlBu10div4}{RGB}{253,174,97}
\definecolor{RdYlBu10div5}{RGB}{254,224,144}
\definecolor{RdYlBu10div6}{RGB}{224,243,248}
\definecolor{RdYlBu10div7}{RGB}{171,217,233}
\definecolor{RdYlBu10div8}{RGB}{116,173,209}
\definecolor{RdYlBu10div9}{RGB}{69,117,180}
\definecolor{RdYlBu10div10}{RGB}{49,54,149}
\definecolor{RdYlGn3div1}{RGB}{252,141,89}
\definecolor{RdYlGn3div2}{RGB}{255,255,191}
\definecolor{RdYlGn3div3}{RGB}{145,207,96}
\definecolor{RdYlGn5div1}{RGB}{215,25,28}
\definecolor{RdYlGn5div2}{RGB}{253,174,97}
\definecolor{RdYlGn5div3}{RGB}{255,255,191}
\definecolor{RdYlGn5div4}{RGB}{166,217,106}
\definecolor{RdYlGn5div5}{RGB}{26,150,65}
\definecolor{RdYlGn7div1}{RGB}{215,48,39}
\definecolor{RdYlGn7div2}{RGB}{252,141,89}
\definecolor{RdYlGn7div3}{RGB}{254,224,139}
\definecolor{RdYlGn7div4}{RGB}{255,255,191}
\definecolor{RdYlGn7div5}{RGB}{217,239,139}
\definecolor{RdYlGn7div6}{RGB}{145,207,96}
\definecolor{RdYlGn7div7}{RGB}{26,152,80}
\definecolor{RdYlGn9div1}{RGB}{215,48,39}
\definecolor{RdYlGn9div2}{RGB}{244,109,67}
\definecolor{RdYlGn9div3}{RGB}{253,174,97}
\definecolor{RdYlGn9div4}{RGB}{254,224,139}
\definecolor{RdYlGn9div5}{RGB}{255,255,191}
\definecolor{RdYlGn9div6}{RGB}{217,239,139}
\definecolor{RdYlGn9div7}{RGB}{166,217,106}
\definecolor{RdYlGn9div8}{RGB}{102,189,99}
\definecolor{RdYlGn9div9}{RGB}{26,152,80}
\definecolor{RdYlGn11div1}{RGB}{165,0,38}
\definecolor{RdYlGn11div2}{RGB}{215,48,39}
\definecolor{RdYlGn11div3}{RGB}{244,109,67}
\definecolor{RdYlGn11div4}{RGB}{253,174,97}
\definecolor{RdYlGn11div5}{RGB}{254,224,139}
\definecolor{RdYlGn11div6}{RGB}{255,255,191}
\definecolor{RdYlGn11div7}{RGB}{217,239,139}
\definecolor{RdYlGn11div8}{RGB}{166,217,106}
\definecolor{RdYlGn11div9}{RGB}{102,189,99}
\definecolor{RdYlGn11div10}{RGB}{26,152,80}
\definecolor{RdYlGn11div11}{RGB}{0,104,55}
\definecolor{Set14qual1}{RGB}{228,26,28}
\definecolor{Set14qual2}{RGB}{55,126,184}
\definecolor{Set14qual3}{RGB}{77,175,74}
\definecolor{Set14qual4}{RGB}{152,78,163}
\definecolor{Set16qual1}{RGB}{228,26,28}
\definecolor{Set16qual2}{RGB}{55,126,184}
\definecolor{Set16qual3}{RGB}{77,175,74}
\definecolor{Set16qual4}{RGB}{152,78,163}
\definecolor{Set16qual5}{RGB}{255,127,0}
\definecolor{Set16qual6}{RGB}{255,255,51}
\definecolor{Set18qual1}{RGB}{228,26,28}
\definecolor{Set18qual2}{RGB}{55,126,184}
\definecolor{Set18qual3}{RGB}{77,175,74}
\definecolor{Set18qual4}{RGB}{152,78,163}
\definecolor{Set18qual5}{RGB}{255,127,0}
\definecolor{Set18qual6}{RGB}{255,255,51}
\definecolor{Set18qual7}{RGB}{166,86,40}
\definecolor{Set18qual8}{RGB}{247,129,191}
\definecolor{Set23qual1}{RGB}{102,194,165}
\definecolor{Set23qual2}{RGB}{252,141,98}
\definecolor{Set23qual3}{RGB}{141,160,203}
\definecolor{Set25qual1}{RGB}{102,194,165}
\definecolor{Set25qual2}{RGB}{252,141,98}
\definecolor{Set25qual3}{RGB}{141,160,203}
\definecolor{Set25qual4}{RGB}{231,138,195}
\definecolor{Set25qual5}{RGB}{166,216,84}
\definecolor{Set27qual1}{RGB}{102,194,165}
\definecolor{Set27qual2}{RGB}{252,141,98}
\definecolor{Set27qual3}{RGB}{141,160,203}
\definecolor{Set27qual4}{RGB}{231,138,195}
\definecolor{Set27qual5}{RGB}{166,216,84}
\definecolor{Set27qual6}{RGB}{255,217,47}
\definecolor{Set27qual7}{RGB}{229,196,148}
\definecolor{Set33qual1}{RGB}{141,211,199}
\definecolor{Set33qual2}{RGB}{255,255,179}
\definecolor{Set33qual3}{RGB}{190,186,218}
\definecolor{Set35qual1}{RGB}{141,211,199}
\definecolor{Set35qual2}{RGB}{255,255,179}
\definecolor{Set35qual3}{RGB}{190,186,218}
\definecolor{Set35qual4}{RGB}{251,128,114}
\definecolor{Set35qual5}{RGB}{128,177,211}
\definecolor{Set37qual1}{RGB}{141,211,199}
\definecolor{Set37qual2}{RGB}{255,255,179}
\definecolor{Set37qual3}{RGB}{190,186,218}
\definecolor{Set37qual4}{RGB}{251,128,114}
\definecolor{Set37qual5}{RGB}{128,177,211}
\definecolor{Set37qual6}{RGB}{253,180,98}
\definecolor{Set37qual7}{RGB}{179,222,105}
\definecolor{Set39qual1}{RGB}{141,211,199}
\definecolor{Set39qual2}{RGB}{255,255,179}
\definecolor{Set39qual3}{RGB}{190,186,218}
\definecolor{Set39qual4}{RGB}{251,128,114}
\definecolor{Set39qual5}{RGB}{128,177,211}
\definecolor{Set39qual6}{RGB}{253,180,98}
\definecolor{Set39qual7}{RGB}{179,222,105}
\definecolor{Set39qual8}{RGB}{252,205,229}
\definecolor{Set39qual9}{RGB}{217,217,217}
\definecolor{Set311qual1}{RGB}{141,211,199}
\definecolor{Set311qual2}{RGB}{255,255,179}
\definecolor{Set311qual3}{RGB}{190,186,218}
\definecolor{Set311qual4}{RGB}{251,128,114}
\definecolor{Set311qual5}{RGB}{128,177,211}
\definecolor{Set311qual6}{RGB}{253,180,98}
\definecolor{Set311qual7}{RGB}{179,222,105}
\definecolor{Set311qual8}{RGB}{252,205,229}
\definecolor{Set311qual9}{RGB}{217,217,217}
\definecolor{Set311qual10}{RGB}{188,128,189}
\definecolor{Set311qual11}{RGB}{204,235,197}
\definecolor{Spectral3div1}{RGB}{252,141,89}
\definecolor{Spectral3div2}{RGB}{255,255,191}
\definecolor{Spectral3div3}{RGB}{153,213,148}
\definecolor{Spectral5div1}{RGB}{215,25,28}
\definecolor{Spectral5div2}{RGB}{253,174,97}
\definecolor{Spectral5div3}{RGB}{255,255,191}
\definecolor{Spectral5div4}{RGB}{171,221,164}
\definecolor{Spectral5div5}{RGB}{43,131,186}
\definecolor{Spectral7div1}{RGB}{213,62,79}
\definecolor{Spectral7div2}{RGB}{252,141,89}
\definecolor{Spectral7div3}{RGB}{254,224,139}
\definecolor{Spectral7div4}{RGB}{255,255,191}
\definecolor{Spectral7div5}{RGB}{230,245,152}
\definecolor{Spectral7div6}{RGB}{153,213,148}
\definecolor{Spectral7div7}{RGB}{50,136,189}
\definecolor{Spectral9div1}{RGB}{213,62,79}
\definecolor{Spectral9div2}{RGB}{244,109,67}
\definecolor{Spectral9div3}{RGB}{253,174,97}
\definecolor{Spectral9div4}{RGB}{254,224,139}
\definecolor{Spectral9div5}{RGB}{255,255,191}
\definecolor{Spectral9div6}{RGB}{230,245,152}
\definecolor{Spectral9div7}{RGB}{171,221,164}
\definecolor{Spectral9div8}{RGB}{102,194,165}
\definecolor{Spectral9div9}{RGB}{50,136,189}
\definecolor{Spectral11div1}{RGB}{158,1,66}
\definecolor{Spectral11div2}{RGB}{213,62,79}
\definecolor{Spectral11div3}{RGB}{244,109,67}
\definecolor{Spectral11div4}{RGB}{253,174,97}
\definecolor{Spectral11div5}{RGB}{254,224,139}
\definecolor{Spectral11div6}{RGB}{255,255,191}
\definecolor{Spectral11div7}{RGB}{230,245,152}
\definecolor{Spectral11div8}{RGB}{171,221,164}
\definecolor{Spectral11div9}{RGB}{102,194,165}
\definecolor{Spectral11div10}{RGB}{50,136,189}
\definecolor{Spectral11div11}{RGB}{94,79,162}
\definecolor{YlGn4seq1}{RGB}{255,255,204}
\definecolor{YlGn4seq2}{RGB}{194,230,153}
\definecolor{YlGn4seq3}{RGB}{120,198,121}
\definecolor{YlGn4seq4}{RGB}{35,132,67}
\definecolor{YlGn6seq1}{RGB}{255,255,204}
\definecolor{YlGn6seq2}{RGB}{217,240,163}
\definecolor{YlGn6seq3}{RGB}{173,221,142}
\definecolor{YlGn6seq4}{RGB}{120,198,121}
\definecolor{YlGn6seq5}{RGB}{49,163,84}
\definecolor{YlGn6seq6}{RGB}{0,104,55}
\definecolor{YlGn8seq1}{RGB}{255,255,229}
\definecolor{YlGn8seq2}{RGB}{247,252,185}
\definecolor{YlGn8seq3}{RGB}{217,240,163}
\definecolor{YlGn8seq4}{RGB}{173,221,142}
\definecolor{YlGn8seq5}{RGB}{120,198,121}
\definecolor{YlGn8seq6}{RGB}{65,171,93}
\definecolor{YlGn8seq7}{RGB}{35,132,67}
\definecolor{YlGn8seq8}{RGB}{0,90,50}
\definecolor{YlGnBu3seq1}{RGB}{237,248,177}
\definecolor{YlGnBu3seq2}{RGB}{127,205,187}
\definecolor{YlGnBu3seq3}{RGB}{44,127,184}
\definecolor{YlGnBu5seq1}{RGB}{255,255,204}
\definecolor{YlGnBu5seq2}{RGB}{161,218,180}
\definecolor{YlGnBu5seq3}{RGB}{65,182,196}
\definecolor{YlGnBu5seq4}{RGB}{44,127,184}
\definecolor{YlGnBu5seq5}{RGB}{37,52,148}
\definecolor{YlGnBu7seq1}{RGB}{255,255,204}
\definecolor{YlGnBu7seq2}{RGB}{199,233,180}
\definecolor{YlGnBu7seq3}{RGB}{127,205,187}
\definecolor{YlGnBu7seq4}{RGB}{65,182,196}
\definecolor{YlGnBu7seq5}{RGB}{29,145,192}
\definecolor{YlGnBu7seq6}{RGB}{34,94,168}
\definecolor{YlGnBu7seq7}{RGB}{12,44,132}
\definecolor{YlGnBu9seq1}{RGB}{255,255,217}
\definecolor{YlGnBu9seq2}{RGB}{237,248,177}
\definecolor{YlGnBu9seq3}{RGB}{199,233,180}
\definecolor{YlGnBu9seq4}{RGB}{127,205,187}
\definecolor{YlGnBu9seq5}{RGB}{65,182,196}
\definecolor{YlGnBu9seq6}{RGB}{29,145,192}
\definecolor{YlGnBu9seq7}{RGB}{34,94,168}
\definecolor{YlGnBu9seq8}{RGB}{37,52,148}
\definecolor{YlGnBu9seq9}{RGB}{8,29,88}
\definecolor{YlOrBr4seq1}{RGB}{255,255,212}
\definecolor{YlOrBr4seq2}{RGB}{254,217,142}
\definecolor{YlOrBr4seq3}{RGB}{254,153,41}
\definecolor{YlOrBr4seq4}{RGB}{204,76,2}
\definecolor{YlOrBr6seq1}{RGB}{255,255,212}
\definecolor{YlOrBr6seq2}{RGB}{254,227,145}
\definecolor{YlOrBr6seq3}{RGB}{254,196,79}
\definecolor{YlOrBr6seq4}{RGB}{254,153,41}
\definecolor{YlOrBr6seq5}{RGB}{217,95,14}
\definecolor{YlOrBr6seq6}{RGB}{153,52,4}
\definecolor{YlOrBr8seq1}{RGB}{255,255,229}
\definecolor{YlOrBr8seq2}{RGB}{255,247,188}
\definecolor{YlOrBr8seq3}{RGB}{254,227,145}
\definecolor{YlOrBr8seq4}{RGB}{254,196,79}
\definecolor{YlOrBr8seq5}{RGB}{254,153,41}
\definecolor{YlOrBr8seq6}{RGB}{236,112,20}
\definecolor{YlOrBr8seq7}{RGB}{204,76,2}
\definecolor{YlOrBr8seq8}{RGB}{140,45,4}
\definecolor{YlOrRd3seq1}{RGB}{255,237,160}
\definecolor{YlOrRd3seq2}{RGB}{254,178,76}
\definecolor{YlOrRd3seq3}{RGB}{240,59,32}
\definecolor{YlOrRd5seq1}{RGB}{255,255,178}
\definecolor{YlOrRd5seq2}{RGB}{254,204,92}
\definecolor{YlOrRd5seq3}{RGB}{253,141,60}
\definecolor{YlOrRd5seq4}{RGB}{240,59,32}
\definecolor{YlOrRd5seq5}{RGB}{189,0,38}
\definecolor{YlOrRd7seq1}{RGB}{255,255,178}
\definecolor{YlOrRd7seq2}{RGB}{254,217,118}
\definecolor{YlOrRd7seq3}{RGB}{254,178,76}
\definecolor{YlOrRd7seq4}{RGB}{253,141,60}
\definecolor{YlOrRd7seq5}{RGB}{252,78,42}
\definecolor{YlOrRd7seq6}{RGB}{227,26,28}
\definecolor{YlOrRd7seq7}{RGB}{177,0,38}
\definecolor{YlOrRd9seq1}{RGB}{255,255,204}
\definecolor{YlOrRd9seq2}{RGB}{255,237,160}
\definecolor{YlOrRd9seq3}{RGB}{254,217,118}
\definecolor{YlOrRd9seq4}{RGB}{254,178,76}
\definecolor{YlOrRd9seq5}{RGB}{253,141,60}
\definecolor{YlOrRd9seq6}{RGB}{252,78,42}
\definecolor{YlOrRd9seq7}{RGB}{227,26,28}
\definecolor{YlOrRd9seq8}{RGB}{189,0,38}
\definecolor{YlOrRd9seq9}{RGB}{128,0,38}
\pgfplotsset{/pgfplots/colormap={Accent3qual}{
	rgb255=(127,201,127)
	rgb255=(190,174,212)
	rgb255=(253,192,134)
}}
\pgfplotsset{/pgfplots/colormap={Accent5qual}{
	rgb255=(127,201,127)
	rgb255=(190,174,212)
	rgb255=(253,192,134)
	rgb255=(255,255,153)
	rgb255=(56,108,176)
}}
\pgfplotsset{/pgfplots/colormap={Accent7qual}{
	rgb255=(127,201,127)
	rgb255=(190,174,212)
	rgb255=(253,192,134)
	rgb255=(255,255,153)
	rgb255=(56,108,176)
	rgb255=(240,2,127)
	rgb255=(191,91,23)
}}
\pgfplotsset{/pgfplots/colormap={Blues3seq}{
	rgb255=(222,235,247)
	rgb255=(158,202,225)
	rgb255=(49,130,189)
}}
\pgfplotsset{/pgfplots/colormap={Blues5seq}{
	rgb255=(239,243,255)
	rgb255=(189,215,231)
	rgb255=(107,174,214)
	rgb255=(49,130,189)
	rgb255=(8,81,156)
}}
\pgfplotsset{/pgfplots/colormap={Blues7seq}{
	rgb255=(239,243,255)
	rgb255=(198,219,239)
	rgb255=(158,202,225)
	rgb255=(107,174,214)
	rgb255=(66,146,198)
	rgb255=(33,113,181)
	rgb255=(8,69,148)
}}
\pgfplotsset{/pgfplots/colormap={Blues9seq}{
	rgb255=(247,251,255)
	rgb255=(222,235,247)
	rgb255=(198,219,239)
	rgb255=(158,202,225)
	rgb255=(107,174,214)
	rgb255=(66,146,198)
	rgb255=(33,113,181)
	rgb255=(8,81,156)
	rgb255=(8,48,107)
}}
\pgfplotsset{/pgfplots/colormap={BrBG4div}{
	rgb255=(166,97,26)
	rgb255=(223,194,125)
	rgb255=(128,205,193)
	rgb255=(1,133,113)
}}
\pgfplotsset{/pgfplots/colormap={BrBG6div}{
	rgb255=(140,81,10)
	rgb255=(216,179,101)
	rgb255=(246,232,195)
	rgb255=(199,234,229)
	rgb255=(90,180,172)
	rgb255=(1,102,94)
}}
\pgfplotsset{/pgfplots/colormap={BrBG8div}{
	rgb255=(140,81,10)
	rgb255=(191,129,45)
	rgb255=(223,194,125)
	rgb255=(246,232,195)
	rgb255=(199,234,229)
	rgb255=(128,205,193)
	rgb255=(53,151,143)
	rgb255=(1,102,94)
}}
\pgfplotsset{/pgfplots/colormap={BrBG10div}{
	rgb255=(84,48,5)
	rgb255=(140,81,10)
	rgb255=(191,129,45)
	rgb255=(223,194,125)
	rgb255=(246,232,195)
	rgb255=(199,234,229)
	rgb255=(128,205,193)
	rgb255=(53,151,143)
	rgb255=(1,102,94)
	rgb255=(0,60,48)
}}
\pgfplotsset{/pgfplots/colormap={BuGn3seq}{
	rgb255=(229,245,249)
	rgb255=(153,216,201)
	rgb255=(44,162,95)
}}
\pgfplotsset{/pgfplots/colormap={BuGn5seq}{
	rgb255=(237,248,251)
	rgb255=(178,226,226)
	rgb255=(102,194,164)
	rgb255=(44,162,95)
	rgb255=(0,109,44)
}}
\pgfplotsset{/pgfplots/colormap={BuGn7seq}{
	rgb255=(237,248,251)
	rgb255=(204,236,230)
	rgb255=(153,216,201)
	rgb255=(102,194,164)
	rgb255=(65,174,118)
	rgb255=(35,139,69)
	rgb255=(0,88,36)
}}
\pgfplotsset{/pgfplots/colormap={BuGn9seq}{
	rgb255=(247,252,253)
	rgb255=(229,245,249)
	rgb255=(204,236,230)
	rgb255=(153,216,201)
	rgb255=(102,194,164)
	rgb255=(65,174,118)
	rgb255=(35,139,69)
	rgb255=(0,109,44)
	rgb255=(0,68,27)
}}
\pgfplotsset{/pgfplots/colormap={BuPu4seq}{
	rgb255=(237,248,251)
	rgb255=(179,205,227)
	rgb255=(140,150,198)
	rgb255=(136,65,157)
}}
\pgfplotsset{/pgfplots/colormap={BuPu6seq}{
	rgb255=(237,248,251)
	rgb255=(191,211,230)
	rgb255=(158,188,218)
	rgb255=(140,150,198)
	rgb255=(136,86,167)
	rgb255=(129,15,124)
}}
\pgfplotsset{/pgfplots/colormap={BuPu8seq}{
	rgb255=(247,252,253)
	rgb255=(224,236,244)
	rgb255=(191,211,230)
	rgb255=(158,188,218)
	rgb255=(140,150,198)
	rgb255=(140,107,177)
	rgb255=(136,65,157)
	rgb255=(110,1,107)
}}
\pgfplotsset{/pgfplots/colormap={Dark23qual}{
	rgb255=(27,158,119)
	rgb255=(217,95,2)
	rgb255=(117,112,179)
}}
\pgfplotsset{/pgfplots/colormap={Dark25qual}{
	rgb255=(27,158,119)
	rgb255=(217,95,2)
	rgb255=(117,112,179)
	rgb255=(231,41,138)
	rgb255=(102,166,30)
}}
\pgfplotsset{/pgfplots/colormap={Dark27qual}{
	rgb255=(27,158,119)
	rgb255=(217,95,2)
	rgb255=(117,112,179)
	rgb255=(231,41,138)
	rgb255=(102,166,30)
	rgb255=(230,171,2)
	rgb255=(166,118,29)
}}
\pgfplotsset{/pgfplots/colormap={GnBu3seq}{
	rgb255=(224,243,219)
	rgb255=(168,221,181)
	rgb255=(67,162,202)
}}
\pgfplotsset{/pgfplots/colormap={GnBu5seq}{
	rgb255=(240,249,232)
	rgb255=(186,228,188)
	rgb255=(123,204,196)
	rgb255=(67,162,202)
	rgb255=(8,104,172)
}}
\pgfplotsset{/pgfplots/colormap={GnBu7seq}{
	rgb255=(240,249,232)
	rgb255=(204,235,197)
	rgb255=(168,221,181)
	rgb255=(123,204,196)
	rgb255=(78,179,211)
	rgb255=(43,140,190)
	rgb255=(8,88,158)
}}
\pgfplotsset{/pgfplots/colormap={GnBu9seq}{
	rgb255=(247,252,240)
	rgb255=(224,243,219)
	rgb255=(204,235,197)
	rgb255=(168,221,181)
	rgb255=(123,204,196)
	rgb255=(78,179,211)
	rgb255=(43,140,190)
	rgb255=(8,104,172)
	rgb255=(8,64,129)
}}
\pgfplotsset{/pgfplots/colormap={Greens4seq}{
	rgb255=(237,248,233)
	rgb255=(186,228,179)
	rgb255=(116,196,118)
	rgb255=(35,139,69)
}}
\pgfplotsset{/pgfplots/colormap={Greens6seq}{
	rgb255=(237,248,233)
	rgb255=(199,233,192)
	rgb255=(161,217,155)
	rgb255=(116,196,118)
	rgb255=(49,163,84)
	rgb255=(0,109,44)
}}
\pgfplotsset{/pgfplots/colormap={Greens8seq}{
	rgb255=(247,252,245)
	rgb255=(229,245,224)
	rgb255=(199,233,192)
	rgb255=(161,217,155)
	rgb255=(116,196,118)
	rgb255=(65,171,93)
	rgb255=(35,139,69)
	rgb255=(0,90,50)
}}
\pgfplotsset{/pgfplots/colormap={Greys3seq}{
	rgb255=(240,240,240)
	rgb255=(189,189,189)
	rgb255=(99,99,99)
}}
\pgfplotsset{/pgfplots/colormap={Greys5seq}{
	rgb255=(247,247,247)
	rgb255=(204,204,204)
	rgb255=(150,150,150)
	rgb255=(99,99,99)
	rgb255=(37,37,37)
}}
\pgfplotsset{/pgfplots/colormap={Greys7seq}{
	rgb255=(247,247,247)
	rgb255=(217,217,217)
	rgb255=(189,189,189)
	rgb255=(150,150,150)
	rgb255=(115,115,115)
	rgb255=(82,82,82)
	rgb255=(37,37,37)
}}
\pgfplotsset{/pgfplots/colormap={Greys9seq}{
	rgb255=(255,255,255)
	rgb255=(240,240,240)
	rgb255=(217,217,217)
	rgb255=(189,189,189)
	rgb255=(150,150,150)
	rgb255=(115,115,115)
	rgb255=(82,82,82)
	rgb255=(37,37,37)
	rgb255=(0,0,0)
}}
\pgfplotsset{/pgfplots/colormap={Oranges4seq}{
	rgb255=(254,237,222)
	rgb255=(253,190,133)
	rgb255=(253,141,60)
	rgb255=(217,71,1)
}}
\pgfplotsset{/pgfplots/colormap={Oranges6seq}{
	rgb255=(254,237,222)
	rgb255=(253,208,162)
	rgb255=(253,174,107)
	rgb255=(253,141,60)
	rgb255=(230,85,13)
	rgb255=(166,54,3)
}}
\pgfplotsset{/pgfplots/colormap={Oranges8seq}{
	rgb255=(255,245,235)
	rgb255=(254,230,206)
	rgb255=(253,208,162)
	rgb255=(253,174,107)
	rgb255=(253,141,60)
	rgb255=(241,105,19)
	rgb255=(217,72,1)
	rgb255=(140,45,4)
}}
\pgfplotsset{/pgfplots/colormap={OrRd3seq}{
	rgb255=(254,232,200)
	rgb255=(253,187,132)
	rgb255=(227,74,51)
}}
\pgfplotsset{/pgfplots/colormap={OrRd5seq}{
	rgb255=(254,240,217)
	rgb255=(253,204,138)
	rgb255=(252,141,89)
	rgb255=(227,74,51)
	rgb255=(179,0,0)
}}
\pgfplotsset{/pgfplots/colormap={OrRd7seq}{
	rgb255=(254,240,217)
	rgb255=(253,212,158)
	rgb255=(253,187,132)
	rgb255=(252,141,89)
	rgb255=(239,101,72)
	rgb255=(215,48,31)
	rgb255=(153,0,0)
}}
\pgfplotsset{/pgfplots/colormap={OrRd9seq}{
	rgb255=(255,247,236)
	rgb255=(254,232,200)
	rgb255=(253,212,158)
	rgb255=(253,187,132)
	rgb255=(252,141,89)
	rgb255=(239,101,72)
	rgb255=(215,48,31)
	rgb255=(179,0,0)
	rgb255=(127,0,0)
}}
\pgfplotsset{/pgfplots/colormap={Paired4qual}{
	rgb255=(166,206,227)
	rgb255=(31,120,180)
	rgb255=(178,223,138)
	rgb255=(51,160,44)
}}
\pgfplotsset{/pgfplots/colormap={Paired6qual}{
	rgb255=(166,206,227)
	rgb255=(31,120,180)
	rgb255=(178,223,138)
	rgb255=(51,160,44)
	rgb255=(251,154,153)
	rgb255=(227,26,28)
}}
\pgfplotsset{/pgfplots/colormap={Paired8qual}{
	rgb255=(166,206,227)
	rgb255=(31,120,180)
	rgb255=(178,223,138)
	rgb255=(51,160,44)
	rgb255=(251,154,153)
	rgb255=(227,26,28)
	rgb255=(253,191,111)
	rgb255=(255,127,0)
}}
\pgfplotsset{/pgfplots/colormap={Paired10qual}{
	rgb255=(166,206,227)
	rgb255=(31,120,180)
	rgb255=(178,223,138)
	rgb255=(51,160,44)
	rgb255=(251,154,153)
	rgb255=(227,26,28)
	rgb255=(253,191,111)
	rgb255=(255,127,0)
	rgb255=(202,178,214)
	rgb255=(106,61,154)
}}
\pgfplotsset{/pgfplots/colormap={Paired12qual}{
	rgb255=(166,206,227)
	rgb255=(31,120,180)
	rgb255=(178,223,138)
	rgb255=(51,160,44)
	rgb255=(251,154,153)
	rgb255=(227,26,28)
	rgb255=(253,191,111)
	rgb255=(255,127,0)
	rgb255=(202,178,214)
	rgb255=(106,61,154)
	rgb255=(255,255,153)
	rgb255=(177,89,40)
}}
\pgfplotsset{/pgfplots/colormap={Pastel14qual}{
	rgb255=(251,180,174)
	rgb255=(179,205,227)
	rgb255=(204,235,197)
	rgb255=(222,203,228)
}}
\pgfplotsset{/pgfplots/colormap={Pastel16qual}{
	rgb255=(251,180,174)
	rgb255=(179,205,227)
	rgb255=(204,235,197)
	rgb255=(222,203,228)
	rgb255=(254,217,166)
	rgb255=(255,255,204)
}}
\pgfplotsset{/pgfplots/colormap={Pastel18qual}{
	rgb255=(251,180,174)
	rgb255=(179,205,227)
	rgb255=(204,235,197)
	rgb255=(222,203,228)
	rgb255=(254,217,166)
	rgb255=(255,255,204)
	rgb255=(229,216,189)
	rgb255=(253,218,236)
}}
\pgfplotsset{/pgfplots/colormap={Pastel23qual}{
	rgb255=(179,226,205)
	rgb255=(253,205,172)
	rgb255=(203,213,232)
}}
\pgfplotsset{/pgfplots/colormap={Pastel25qual}{
	rgb255=(179,226,205)
	rgb255=(253,205,172)
	rgb255=(203,213,232)
	rgb255=(244,202,228)
	rgb255=(230,245,201)
}}
\pgfplotsset{/pgfplots/colormap={Pastel27qual}{
	rgb255=(179,226,205)
	rgb255=(253,205,172)
	rgb255=(203,213,232)
	rgb255=(244,202,228)
	rgb255=(230,245,201)
	rgb255=(255,242,174)
	rgb255=(241,226,204)
}}
\pgfplotsset{/pgfplots/colormap={PiYG3div}{
	rgb255=(233,163,201)
	rgb255=(247,247,247)
	rgb255=(161,215,106)
}}
\pgfplotsset{/pgfplots/colormap={PiYG5div}{
	rgb255=(208,28,139)
	rgb255=(241,182,218)
	rgb255=(247,247,247)
	rgb255=(184,225,134)
	rgb255=(77,172,38)
}}
\pgfplotsset{/pgfplots/colormap={PiYG7div}{
	rgb255=(197,27,125)
	rgb255=(233,163,201)
	rgb255=(253,224,239)
	rgb255=(247,247,247)
	rgb255=(230,245,208)
	rgb255=(161,215,106)
	rgb255=(77,146,33)
}}
\pgfplotsset{/pgfplots/colormap={PiYG9div}{
	rgb255=(197,27,125)
	rgb255=(222,119,174)
	rgb255=(241,182,218)
	rgb255=(253,224,239)
	rgb255=(247,247,247)
	rgb255=(230,245,208)
	rgb255=(184,225,134)
	rgb255=(127,188,65)
	rgb255=(77,146,33)
}}
\pgfplotsset{/pgfplots/colormap={PiYG11div}{
	rgb255=(142,1,82)
	rgb255=(197,27,125)
	rgb255=(222,119,174)
	rgb255=(241,182,218)
	rgb255=(253,224,239)
	rgb255=(247,247,247)
	rgb255=(230,245,208)
	rgb255=(184,225,134)
	rgb255=(127,188,65)
	rgb255=(77,146,33)
	rgb255=(39,100,25)
}}
\pgfplotsset{/pgfplots/colormap={PRGn4div}{
	rgb255=(123,50,148)
	rgb255=(194,165,207)
	rgb255=(166,219,160)
	rgb255=(0,136,55)
}}
\pgfplotsset{/pgfplots/colormap={PRGn6div}{
	rgb255=(118,42,131)
	rgb255=(175,141,195)
	rgb255=(231,212,232)
	rgb255=(217,240,211)
	rgb255=(127,191,123)
	rgb255=(27,120,55)
}}
\pgfplotsset{/pgfplots/colormap={PRGn8div}{
	rgb255=(118,42,131)
	rgb255=(153,112,171)
	rgb255=(194,165,207)
	rgb255=(231,212,232)
	rgb255=(217,240,211)
	rgb255=(166,219,160)
	rgb255=(90,174,97)
	rgb255=(27,120,55)
}}
\pgfplotsset{/pgfplots/colormap={PRGn10div}{
	rgb255=(64,0,75)
	rgb255=(118,42,131)
	rgb255=(153,112,171)
	rgb255=(194,165,207)
	rgb255=(231,212,232)
	rgb255=(217,240,211)
	rgb255=(166,219,160)
	rgb255=(90,174,97)
	rgb255=(27,120,55)
	rgb255=(0,68,27)
}}
\pgfplotsset{/pgfplots/colormap={PuBu3seq}{
	rgb255=(236,231,242)
	rgb255=(166,189,219)
	rgb255=(43,140,190)
}}
\pgfplotsset{/pgfplots/colormap={PuBu5seq}{
	rgb255=(241,238,246)
	rgb255=(189,201,225)
	rgb255=(116,169,207)
	rgb255=(43,140,190)
	rgb255=(4,90,141)
}}
\pgfplotsset{/pgfplots/colormap={PuBu7seq}{
	rgb255=(241,238,246)
	rgb255=(208,209,230)
	rgb255=(166,189,219)
	rgb255=(116,169,207)
	rgb255=(54,144,192)
	rgb255=(5,112,176)
	rgb255=(3,78,123)
}}
\pgfplotsset{/pgfplots/colormap={PuBu9seq}{
	rgb255=(255,247,251)
	rgb255=(236,231,242)
	rgb255=(208,209,230)
	rgb255=(166,189,219)
	rgb255=(116,169,207)
	rgb255=(54,144,192)
	rgb255=(5,112,176)
	rgb255=(4,90,141)
	rgb255=(2,56,88)
}}
\pgfplotsset{/pgfplots/colormap={PuBuGn4seq}{
	rgb255=(246,239,247)
	rgb255=(189,201,225)
	rgb255=(103,169,207)
	rgb255=(2,129,138)
}}
\pgfplotsset{/pgfplots/colormap={PuBuGn6seq}{
	rgb255=(246,239,247)
	rgb255=(208,209,230)
	rgb255=(166,189,219)
	rgb255=(103,169,207)
	rgb255=(28,144,153)
	rgb255=(1,108,89)
}}
\pgfplotsset{/pgfplots/colormap={PuBuGn8seq}{
	rgb255=(255,247,251)
	rgb255=(236,226,240)
	rgb255=(208,209,230)
	rgb255=(166,189,219)
	rgb255=(103,169,207)
	rgb255=(54,144,192)
	rgb255=(2,129,138)
	rgb255=(1,100,80)
}}
\pgfplotsset{/pgfplots/colormap={PuOr3div}{
	rgb255=(241,163,64)
	rgb255=(247,247,247)
	rgb255=(153,142,195)
}}
\pgfplotsset{/pgfplots/colormap={PuOr5div}{
	rgb255=(230,97,1)
	rgb255=(253,184,99)
	rgb255=(247,247,247)
	rgb255=(178,171,210)
	rgb255=(94,60,153)
}}
\pgfplotsset{/pgfplots/colormap={PuOr7div}{
	rgb255=(179,88,6)
	rgb255=(241,163,64)
	rgb255=(254,224,182)
	rgb255=(247,247,247)
	rgb255=(216,218,235)
	rgb255=(153,142,195)
	rgb255=(84,39,136)
}}
\pgfplotsset{/pgfplots/colormap={PuOr9div}{
	rgb255=(179,88,6)
	rgb255=(224,130,20)
	rgb255=(253,184,99)
	rgb255=(254,224,182)
	rgb255=(247,247,247)
	rgb255=(216,218,235)
	rgb255=(178,171,210)
	rgb255=(128,115,172)
	rgb255=(84,39,136)
}}
\pgfplotsset{/pgfplots/colormap={PuOr11div}{
	rgb255=(127,59,8)
	rgb255=(179,88,6)
	rgb255=(224,130,20)
	rgb255=(253,184,99)
	rgb255=(254,224,182)
	rgb255=(247,247,247)
	rgb255=(216,218,235)
	rgb255=(178,171,210)
	rgb255=(128,115,172)
	rgb255=(84,39,136)
	rgb255=(45,0,75)
}}
\pgfplotsset{/pgfplots/colormap={PuRd4seq}{
	rgb255=(241,238,246)
	rgb255=(215,181,216)
	rgb255=(223,101,176)
	rgb255=(206,18,86)
}}
\pgfplotsset{/pgfplots/colormap={PuRd6seq}{
	rgb255=(241,238,246)
	rgb255=(212,185,218)
	rgb255=(201,148,199)
	rgb255=(223,101,176)
	rgb255=(221,28,119)
	rgb255=(152,0,67)
}}
\pgfplotsset{/pgfplots/colormap={PuRd8seq}{
	rgb255=(247,244,249)
	rgb255=(231,225,239)
	rgb255=(212,185,218)
	rgb255=(201,148,199)
	rgb255=(223,101,176)
	rgb255=(231,41,138)
	rgb255=(206,18,86)
	rgb255=(145,0,63)
}}
\pgfplotsset{/pgfplots/colormap={Purples3seq}{
	rgb255=(239,237,245)
	rgb255=(188,189,220)
	rgb255=(117,107,177)
}}
\pgfplotsset{/pgfplots/colormap={Purples5seq}{
	rgb255=(242,240,247)
	rgb255=(203,201,226)
	rgb255=(158,154,200)
	rgb255=(117,107,177)
	rgb255=(84,39,143)
}}
\pgfplotsset{/pgfplots/colormap={Purples7seq}{
	rgb255=(242,240,247)
	rgb255=(218,218,235)
	rgb255=(188,189,220)
	rgb255=(158,154,200)
	rgb255=(128,125,186)
	rgb255=(106,81,163)
	rgb255=(74,20,134)
}}
\pgfplotsset{/pgfplots/colormap={Purples9seq}{
	rgb255=(252,251,253)
	rgb255=(239,237,245)
	rgb255=(218,218,235)
	rgb255=(188,189,220)
	rgb255=(158,154,200)
	rgb255=(128,125,186)
	rgb255=(106,81,163)
	rgb255=(84,39,143)
	rgb255=(63,0,125)
}}
\pgfplotsset{/pgfplots/colormap={RdBu4div}{
	rgb255=(202,0,32)
	rgb255=(244,165,130)
	rgb255=(146,197,222)
	rgb255=(5,113,176)
}}
\pgfplotsset{/pgfplots/colormap={RdBu6div}{
	rgb255=(178,24,43)
	rgb255=(239,138,98)
	rgb255=(253,219,199)
	rgb255=(209,229,240)
	rgb255=(103,169,207)
	rgb255=(33,102,172)
}}
\pgfplotsset{/pgfplots/colormap={RdBu8div}{
	rgb255=(178,24,43)
	rgb255=(214,96,77)
	rgb255=(244,165,130)
	rgb255=(253,219,199)
	rgb255=(209,229,240)
	rgb255=(146,197,222)
	rgb255=(67,147,195)
	rgb255=(33,102,172)
}}
\pgfplotsset{/pgfplots/colormap={RdBu10div}{
	rgb255=(103,0,31)
	rgb255=(178,24,43)
	rgb255=(214,96,77)
	rgb255=(244,165,130)
	rgb255=(253,219,199)
	rgb255=(209,229,240)
	rgb255=(146,197,222)
	rgb255=(67,147,195)
	rgb255=(33,102,172)
	rgb255=(5,48,97)
}}
\pgfplotsset{/pgfplots/colormap={RdGy3div}{
	rgb255=(239,138,98)
	rgb255=(255,255,255)
	rgb255=(153,153,153)
}}
\pgfplotsset{/pgfplots/colormap={RdGy5div}{
	rgb255=(202,0,32)
	rgb255=(244,165,130)
	rgb255=(255,255,255)
	rgb255=(186,186,186)
	rgb255=(64,64,64)
}}
\pgfplotsset{/pgfplots/colormap={RdGy7div}{
	rgb255=(178,24,43)
	rgb255=(239,138,98)
	rgb255=(253,219,199)
	rgb255=(255,255,255)
	rgb255=(224,224,224)
	rgb255=(153,153,153)
	rgb255=(77,77,77)
}}
\pgfplotsset{/pgfplots/colormap={RdGy9div}{
	rgb255=(178,24,43)
	rgb255=(214,96,77)
	rgb255=(244,165,130)
	rgb255=(253,219,199)
	rgb255=(255,255,255)
	rgb255=(224,224,224)
	rgb255=(186,186,186)
	rgb255=(135,135,135)
	rgb255=(77,77,77)
}}
\pgfplotsset{/pgfplots/colormap={RdGy11div}{
	rgb255=(103,0,31)
	rgb255=(178,24,43)
	rgb255=(214,96,77)
	rgb255=(244,165,130)
	rgb255=(253,219,199)
	rgb255=(255,255,255)
	rgb255=(224,224,224)
	rgb255=(186,186,186)
	rgb255=(135,135,135)
	rgb255=(77,77,77)
	rgb255=(26,26,26)
}}
\pgfplotsset{/pgfplots/colormap={RdPu4seq}{
	rgb255=(254,235,226)
	rgb255=(251,180,185)
	rgb255=(247,104,161)
	rgb255=(174,1,126)
}}
\pgfplotsset{/pgfplots/colormap={RdPu6seq}{
	rgb255=(254,235,226)
	rgb255=(252,197,192)
	rgb255=(250,159,181)
	rgb255=(247,104,161)
	rgb255=(197,27,138)
	rgb255=(122,1,119)
}}
\pgfplotsset{/pgfplots/colormap={RdPu8seq}{
	rgb255=(255,247,243)
	rgb255=(253,224,221)
	rgb255=(252,197,192)
	rgb255=(250,159,181)
	rgb255=(247,104,161)
	rgb255=(221,52,151)
	rgb255=(174,1,126)
	rgb255=(122,1,119)
}}
\pgfplotsset{/pgfplots/colormap={Reds3seq}{
	rgb255=(254,224,210)
	rgb255=(252,146,114)
	rgb255=(222,45,38)
}}
\pgfplotsset{/pgfplots/colormap={Reds5seq}{
	rgb255=(254,229,217)
	rgb255=(252,174,145)
	rgb255=(251,106,74)
	rgb255=(222,45,38)
	rgb255=(165,15,21)
}}
\pgfplotsset{/pgfplots/colormap={Reds7seq}{
	rgb255=(254,229,217)
	rgb255=(252,187,161)
	rgb255=(252,146,114)
	rgb255=(251,106,74)
	rgb255=(239,59,44)
	rgb255=(203,24,29)
	rgb255=(153,0,13)
}}
\pgfplotsset{/pgfplots/colormap={Reds9seq}{
	rgb255=(255,245,240)
	rgb255=(254,224,210)
	rgb255=(252,187,161)
	rgb255=(252,146,114)
	rgb255=(251,106,74)
	rgb255=(239,59,44)
	rgb255=(203,24,29)
	rgb255=(165,15,21)
	rgb255=(103,0,13)
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu4div}{
	rgb255=(215,25,28)
	rgb255=(253,174,97)
	rgb255=(171,217,233)
	rgb255=(44,123,182)
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu6div}{
	rgb255=(215,48,39)
	rgb255=(252,141,89)
	rgb255=(254,224,144)
	rgb255=(224,243,248)
	rgb255=(145,191,219)
	rgb255=(69,117,180)
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu8div}{
	rgb255=(215,48,39)
	rgb255=(244,109,67)
	rgb255=(253,174,97)
	rgb255=(254,224,144)
	rgb255=(224,243,248)
	rgb255=(171,217,233)
	rgb255=(116,173,209)
	rgb255=(69,117,180)
}}
\pgfplotsset{/pgfplots/colormap={RdYlBu10div}{
	rgb255=(165,0,38)
	rgb255=(215,48,39)
	rgb255=(244,109,67)
	rgb255=(253,174,97)
	rgb255=(254,224,144)
	rgb255=(224,243,248)
	rgb255=(171,217,233)
	rgb255=(116,173,209)
	rgb255=(69,117,180)
	rgb255=(49,54,149)
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn3div}{
	rgb255=(252,141,89)
	rgb255=(255,255,191)
	rgb255=(145,207,96)
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn5div}{
	rgb255=(215,25,28)
	rgb255=(253,174,97)
	rgb255=(255,255,191)
	rgb255=(166,217,106)
	rgb255=(26,150,65)
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn7div}{
	rgb255=(215,48,39)
	rgb255=(252,141,89)
	rgb255=(254,224,139)
	rgb255=(255,255,191)
	rgb255=(217,239,139)
	rgb255=(145,207,96)
	rgb255=(26,152,80)
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn9div}{
	rgb255=(215,48,39)
	rgb255=(244,109,67)
	rgb255=(253,174,97)
	rgb255=(254,224,139)
	rgb255=(255,255,191)
	rgb255=(217,239,139)
	rgb255=(166,217,106)
	rgb255=(102,189,99)
	rgb255=(26,152,80)
}}
\pgfplotsset{/pgfplots/colormap={RdYlGn11div}{
	rgb255=(165,0,38)
	rgb255=(215,48,39)
	rgb255=(244,109,67)
	rgb255=(253,174,97)
	rgb255=(254,224,139)
	rgb255=(255,255,191)
	rgb255=(217,239,139)
	rgb255=(166,217,106)
	rgb255=(102,189,99)
	rgb255=(26,152,80)
	rgb255=(0,104,55)
}}
\pgfplotsset{/pgfplots/colormap={Set14qual}{
	rgb255=(228,26,28)
	rgb255=(55,126,184)
	rgb255=(77,175,74)
	rgb255=(152,78,163)
}}
\pgfplotsset{/pgfplots/colormap={Set16qual}{
	rgb255=(228,26,28)
	rgb255=(55,126,184)
	rgb255=(77,175,74)
	rgb255=(152,78,163)
	rgb255=(255,127,0)
	rgb255=(255,255,51)
}}
\pgfplotsset{/pgfplots/colormap={Set18qual}{
	rgb255=(228,26,28)
	rgb255=(55,126,184)
	rgb255=(77,175,74)
	rgb255=(152,78,163)
	rgb255=(255,127,0)
	rgb255=(255,255,51)
	rgb255=(166,86,40)
	rgb255=(247,129,191)
}}
\pgfplotsset{/pgfplots/colormap={Set23qual}{
	rgb255=(102,194,165)
	rgb255=(252,141,98)
	rgb255=(141,160,203)
}}
\pgfplotsset{/pgfplots/colormap={Set25qual}{
	rgb255=(102,194,165)
	rgb255=(252,141,98)
	rgb255=(141,160,203)
	rgb255=(231,138,195)
	rgb255=(166,216,84)
}}
\pgfplotsset{/pgfplots/colormap={Set27qual}{
	rgb255=(102,194,165)
	rgb255=(252,141,98)
	rgb255=(141,160,203)
	rgb255=(231,138,195)
	rgb255=(166,216,84)
	rgb255=(255,217,47)
	rgb255=(229,196,148)
}}
\pgfplotsset{/pgfplots/colormap={Set33qual}{
	rgb255=(141,211,199)
	rgb255=(255,255,179)
	rgb255=(190,186,218)
}}
\pgfplotsset{/pgfplots/colormap={Set35qual}{
	rgb255=(141,211,199)
	rgb255=(255,255,179)
	rgb255=(190,186,218)
	rgb255=(251,128,114)
	rgb255=(128,177,211)
}}
\pgfplotsset{/pgfplots/colormap={Set37qual}{
	rgb255=(141,211,199)
	rgb255=(255,255,179)
	rgb255=(190,186,218)
	rgb255=(251,128,114)
	rgb255=(128,177,211)
	rgb255=(253,180,98)
	rgb255=(179,222,105)
}}
\pgfplotsset{/pgfplots/colormap={Set39qual}{
	rgb255=(141,211,199)
	rgb255=(255,255,179)
	rgb255=(190,186,218)
	rgb255=(251,128,114)
	rgb255=(128,177,211)
	rgb255=(253,180,98)
	rgb255=(179,222,105)
	rgb255=(252,205,229)
	rgb255=(217,217,217)
}}
\pgfplotsset{/pgfplots/colormap={Set311qual}{
	rgb255=(141,211,199)
	rgb255=(255,255,179)
	rgb255=(190,186,218)
	rgb255=(251,128,114)
	rgb255=(128,177,211)
	rgb255=(253,180,98)
	rgb255=(179,222,105)
	rgb255=(252,205,229)
	rgb255=(217,217,217)
	rgb255=(188,128,189)
	rgb255=(204,235,197)
}}
\pgfplotsset{/pgfplots/colormap={Spectral3div}{
	rgb255=(252,141,89)
	rgb255=(255,255,191)
	rgb255=(153,213,148)
}}
\pgfplotsset{/pgfplots/colormap={Spectral5div}{
	rgb255=(215,25,28)
	rgb255=(253,174,97)
	rgb255=(255,255,191)
	rgb255=(171,221,164)
	rgb255=(43,131,186)
}}
\pgfplotsset{/pgfplots/colormap={Spectral7div}{
	rgb255=(213,62,79)
	rgb255=(252,141,89)
	rgb255=(254,224,139)
	rgb255=(255,255,191)
	rgb255=(230,245,152)
	rgb255=(153,213,148)
	rgb255=(50,136,189)
}}
\pgfplotsset{/pgfplots/colormap={Spectral9div}{
	rgb255=(213,62,79)
	rgb255=(244,109,67)
	rgb255=(253,174,97)
	rgb255=(254,224,139)
	rgb255=(255,255,191)
	rgb255=(230,245,152)
	rgb255=(171,221,164)
	rgb255=(102,194,165)
	rgb255=(50,136,189)
}}
\pgfplotsset{/pgfplots/colormap={Spectral11div}{
	rgb255=(158,1,66)
	rgb255=(213,62,79)
	rgb255=(244,109,67)
	rgb255=(253,174,97)
	rgb255=(254,224,139)
	rgb255=(255,255,191)
	rgb255=(230,245,152)
	rgb255=(171,221,164)
	rgb255=(102,194,165)
	rgb255=(50,136,189)
	rgb255=(94,79,162)
}}
\pgfplotsset{/pgfplots/colormap={YlGn4seq}{
	rgb255=(255,255,204)
	rgb255=(194,230,153)
	rgb255=(120,198,121)
	rgb255=(35,132,67)
}}
\pgfplotsset{/pgfplots/colormap={YlGn6seq}{
	rgb255=(255,255,204)
	rgb255=(217,240,163)
	rgb255=(173,221,142)
	rgb255=(120,198,121)
	rgb255=(49,163,84)
	rgb255=(0,104,55)
}}
\pgfplotsset{/pgfplots/colormap={YlGn8seq}{
	rgb255=(255,255,229)
	rgb255=(247,252,185)
	rgb255=(217,240,163)
	rgb255=(173,221,142)
	rgb255=(120,198,121)
	rgb255=(65,171,93)
	rgb255=(35,132,67)
	rgb255=(0,90,50)
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu3seq}{
	rgb255=(237,248,177)
	rgb255=(127,205,187)
	rgb255=(44,127,184)
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu5seq}{
	rgb255=(255,255,204)
	rgb255=(161,218,180)
	rgb255=(65,182,196)
	rgb255=(44,127,184)
	rgb255=(37,52,148)
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu7seq}{
	rgb255=(255,255,204)
	rgb255=(199,233,180)
	rgb255=(127,205,187)
	rgb255=(65,182,196)
	rgb255=(29,145,192)
	rgb255=(34,94,168)
	rgb255=(12,44,132)
}}
\pgfplotsset{/pgfplots/colormap={YlGnBu9seq}{
	rgb255=(255,255,217)
	rgb255=(237,248,177)
	rgb255=(199,233,180)
	rgb255=(127,205,187)
	rgb255=(65,182,196)
	rgb255=(29,145,192)
	rgb255=(34,94,168)
	rgb255=(37,52,148)
	rgb255=(8,29,88)
}}
\pgfplotsset{/pgfplots/colormap={YlOrBr4seq}{
	rgb255=(255,255,212)
	rgb255=(254,217,142)
	rgb255=(254,153,41)
	rgb255=(204,76,2)
}}
\pgfplotsset{/pgfplots/colormap={YlOrBr6seq}{
	rgb255=(255,255,212)
	rgb255=(254,227,145)
	rgb255=(254,196,79)
	rgb255=(254,153,41)
	rgb255=(217,95,14)
	rgb255=(153,52,4)
}}
\pgfplotsset{/pgfplots/colormap={YlOrBr8seq}{
	rgb255=(255,255,229)
	rgb255=(255,247,188)
	rgb255=(254,227,145)
	rgb255=(254,196,79)
	rgb255=(254,153,41)
	rgb255=(236,112,20)
	rgb255=(204,76,2)
	rgb255=(140,45,4)
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd3seq}{
	rgb255=(255,237,160)
	rgb255=(254,178,76)
	rgb255=(240,59,32)
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd5seq}{
	rgb255=(255,255,178)
	rgb255=(254,204,92)
	rgb255=(253,141,60)
	rgb255=(240,59,32)
	rgb255=(189,0,38)
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd7seq}{
	rgb255=(255,255,178)
	rgb255=(254,217,118)
	rgb255=(254,178,76)
	rgb255=(253,141,60)
	rgb255=(252,78,42)
	rgb255=(227,26,28)
	rgb255=(177,0,38)
}}
\pgfplotsset{/pgfplots/colormap={YlOrRd9seq}{
	rgb255=(255,255,204)
	rgb255=(255,237,160)
	rgb255=(254,217,118)
	rgb255=(254,178,76)
	rgb255=(253,141,60)
	rgb255=(252,78,42)
	rgb255=(227,26,28)
	rgb255=(189,0,38)
	rgb255=(128,0,38)
}}


==> sections/pipeline.tex <==
\section{Typical RT pipeline}\label{sec:pipeline}

%In this section, we briefly document the principal components that can be found in most modern image based ray tracers.
Image based RT, in opposition to shooting and bouncing rays (SBR), ray launching (RL), and other techniques, aims at exactly finding all possible paths between two nodes, that undergo up to a fixed number of interactions with the environment. Here, interactions are either reflections or diffractions on objects, and are computed using Geometrical Optics (GOs) and the Uniform Theory of Diffraction (UTD) \cite{mcnamaraIntroductionUniformGeometrical1990}. Image RT often offers a better accuracy than RL or SBR, but at a higher computational cost.

Modern RT based engines are composed of multiple blocks that altogether form a processing pipeline taking, for instance, a spatial configuration as input, and providing an estimated received electromagnetic (EM) field at the output (Fig \ref{fig:pipeline}). Regardless of the RT technique, most implementations share common steps in their working process \cite{yunRayTracingRadio2015,espostiRayTracingTechniques2021,fuschiniRayTracingPropagation2015,egea-lopezOpalOpenSource2021}. The first element is often dedicated to preprocess the input geometry, thus making sure it contains necessary information, such as surface normal computation. In the frame of this paper, we assume that the 3-D scene (made of objects) can be described as a collection of $N$ facets, with the surface of each faced represented by an implicit equation, and edges are defined as the intersection between pairs of facets. A second step consists in determining the so-called $N$-by-$N$ visibility matrix $\mathcal{V}$, whose "$ij$"-th binary entry is 1 if the $i$-th object is visible to the $j$-th, and 0 otherwise. As a third step, the path finding component estimates, for each pair BS-UE, all the possible paths. Finally, the paths are used to compute the EM fields at the different UE locations.

\begin{figure}[t]
    \scriptsize
    \centering
    \begin{tikzpicture}
        \newcommand\nodedistance{0.4cm}
            \node[block] (geom) at (0,0) {Scene\\geometry\\construction};

            \node[block] (visibility) at (3,0) {Visibility\\matrix};
            \node[block] (path) at (3,-2) {Path finding};
            \node[block] (em) at (0,-2) {EM fields};
            \draw[<-,thick] (geom.west) -- ++(-\nodedistance,0) node[left,align=center] {Geometrical\\input files};
            \draw[->, thick] (geom.east) -- (visibility.west);
            \draw[->, thick] (visibility.south) -- (path.north);
            \draw[<-, thick] (visibility.north) |- ++(-\nodedistance,\nodedistance) node[left, align=center] {BS location};
            \draw[<-, thick] (path.south) -- ++(0, -\nodedistance) node[below, align=center] {UE locations};
            \draw[->, thick] (path.west) -- (em.east) node[midway] (midway) {};
            \draw[->, thick] (midway.center) |- ([yshift=-\nodedistance]em.south) node[left, align=center] {All rays from\\BS to UEs};
            \draw[->, thick] (em.west) -- ++(-\nodedistance, 0) node[left, align=center] {EM field at\\UE locations};

        \end{tikzpicture}
        \caption{High-level view of the typical blocks that constitute modern ray tracers. Some blocks can be further divided into smaller tasks, such as the geometry construction, or some may be processed altogether to improve performance, such as for the path finding and EM fields computation \cite{egea-lopezOpalOpenSource2021}.}
        \label{fig:pipeline}
    \end{figure}

    \subsection{Scene geometry construction}
    Performing RT requires a detailed and appropriate description of the environment to better simulate the transport of rays. For outdoor propagation, one can use publicly available datasets, \eg from OpenStreetMap\footnote{OverPass Turbo from Martin Reifer: \url{https://overpass-turbo.eu/}} for the position and shapes of buildings, and from NASA\footnote{USGS Earth Explorer: \url{https://earthexplorer.usgs.gov/}} for terrain elevation. It is also common to combine open data and CAD programs to construct a detailed geometry \cite{egea-lopezOpalOpenSource2021}. It is also important to use efficient data structures, such as KdTrees \cite{waldBuildingFastKdTrees2006}, to reduce the overall computational time. Generally speaking, the scene geometry construction step embraces most preprocessing that is required for future blocks to work.

    \subsection{Visibility matrix}
    RT derives all possible paths between the BS and UEs by testing if a path is physically possible, for every combination of facets or edges in the geometry. As the number of combinations can become dramatically large, it is common to prune some of these combinations before they are actually tested. This is performed by building the visibility matrix, $\mathcal{V}$, that encodes, for every facet, the list of facets it can see\cite{chandakFastAccurateGeometric2011}. As $\mathcal{V}$ is usually sparse (as in Fig. \ref{eq:adjacency}), due to objects in the scene shadowing each other, we can significantly reduce the amount of paths to be tested.

    \subsection{Path finding}\label{sec:path_finding}

    The path finding step is a function that takes as input both BS and UE(s) locations, and a list of surfaces or edges with which we would like to have pre-defined interactions, and returns as output the list of interaction points. This list of points is such that is satisfies the laws of reflection and diffraction. Then, the path goes through a validation process that verifies that no line segment within the path is obstructed by any object or if interaction points actually lie within the corresponding facets or edges.

    \subsection{Electromagnetic fields}

    Once all paths are determined, the EM field can be computed at every UE location using, for example, the GOs and UTD to evaluate reflection and diffraction coefficients. Even though separating path finding and EM fields steps allows for a more simplified implementation, it can be preferred to perform both simultaneously \cite{egea-lopezOpalOpenSource2021} to avoid storing all the paths.

